Rethinking ASTE: A Minimalist Tagging Scheme Alongside Contrastive Learning

Aspect Sentiment Triplet Extraction (ASTE) is a burgeoning subtask of fine-grained sentiment analysis, aiming to extract structured sentiment triplets from unstructured textual data. Existing approaches to ASTE often complicate the task with additional structures or external data. In this research, we propose a novel tagging scheme and employ a contrastive learning approach to mitigate these challenges. The proposed approach demonstrates comparable or superior performance in comparison to state-of-the-art techniques, while featuring a more compact design and reduced computational overhead. Notably, even in the era of Large Language Models (LLMs), our method exhibits superior efficacy compared to GPT 3.5 and GPT 4 in a few-shot learning scenarios. This study also provides valuable insights for the advancement of ASTE techniques within the paradigm of large language models.

==> ___misc.tex <==
% This paper presents Aspect Sentiment Triplet Extraction (ASTE) as a subtask of fine-grained sentiment analysis, aiming to extract (Aspect, Opinion, Sentiment) triplets from unstructured text. Existing ASTE methods often introduce unnecessary complexity, such as additional structures or external information. To address this issue, we propose a redesigned tagging scheme and a contrastive learning approach. The proposed method achieves comparable or superior performance to state-of-the-art techniques, with a smaller design and lower computational cost. Even in the era of large language models, our method outperforms GPT3.5 and GPT4. This study provides valuable insights for ASTE in the context of large language models.


% Aspect Sentiment Triplet Extraction (ASTE) is a burgeoning subtask within the domain of fine-grained sentiment analysis, which aims to extract all the (Aspect, Opinion, Sentiment) triplets from unstructured textual data. Existing approaches to ASTE can be broadly categorized into two paradigms: those treating it as an understanding problem and those treating it as a generation problem. The former predominantly leverage pre-trained language models (PLMs) and classification heads.

% However, these approaches often introduce superfluous and intricate structures, such as additional classification heads or external information, in order to achieve improved performance. This paper posits that the fundamental issue lies in the conical context representation of PLMs and the lack of conciseness in the employed tagging scheme, resulting in challenges associated with learning the classification heads.

% To address this concern, the paper presents a reimagined tagging scheme that, based on theoretical analysis, minimizes the number of labels, thereby facilitating the classification of the heads. Furthermore, a contrastive learning method is devised to enhance the distribution of word vectors produced by PLMs.

% Through these innovations, the proposed methodology achieves performance levels comparable to, or even surpassing, the state-of-the-art techniques, while featuring a more streamlined classification head design and reduced computational overhead. These findings offer valuable insights for resolving the ASTE problem.

% It is noteworthy that, even in the era of large-scale language models, the proposed approach demonstrates superior efficacy and efficiency when compared to GPT3.5 and GPT4. This underscores the continued relevance of our method as one of the premier solutions for ASTE in the era of large language models.


% % 引入和介绍问题
% Aspect Sentiment Triplet Extraction (ASTE), an emerging subtask of fine-grained sentiment analysis, \textcolor{red}{emulates} to extract all the \texttt{(Aspect, Opinion, Sentiment)} triplets from an unstructured text. 
% % 现状简介
% % 当前的方法有两类，把ASTE看成理解问题或生成问题。其中，理解式多数基于PLM和分类头。

% % 当前方法的诟病
% % 但是，这些方法往往引入了过多不必要的复杂结构（分类头）或外部信息来达到更好的表现。

% % 问题根源
% % 本文认为问题的根本在于PLM的圆锥形上下文表征和tagging scheme不够精简导致的分类头难学。

% Recent methods commonly utilize pretrained language models (PLMs) to encode input text. However, most PLM-based methods have long neglected the conical embedding distribution issue. 

% % 本文的贡献
% % 基于理论分析，我们重新设计了tagging scheme，其不仅采取了目前为止可比方法中最少的标签分类，从而易于分类头分类，而且在此基础上进一步设计了一种对比学习，从而改进了PLM输出词向量的分布。

% % of disregard the cone-shaped embedding distribution issue, constraining PLMs' potential in downstream tasks and hence relying on intricate techniques to leverage the performance, including but not limited to complex architecture design and external information enhancements.

% % 结果
% % 经过这样的改进，我们方法在更小的分类头设计、更低开销的基础上取得了可比甚至高于sota的表现，为解决ASTE问题提供了本质的思考。

% % GPT 时代的问题
% % 值得注意的是，即使在大语言模型时代，我们的方法仍被证明在精确度和效率上超过GPT3.5和4的表现。这表明我们的方法在大语言模型时代仍然是ASTE的最佳解决方案之一。




\begin{comment}
% Aspect sentiment Triplet Extraction (ASTE) is a remarkable and emergent fine-grained sentiment analysis in an aspect-based manner, which is challenging for the difficulty to simultaneously extract an \texttt{(Aspect, Sentiment, Opinion)} triplet accurately from an unstructured text. Despite the substantial advance in Pretrained Language Models (PLMs), the conical 


% 引入和介绍问题
Aspect Sentiment Triplet Extraction (ASTE), an emerging subtask of fine-grained sentiment analysis, \textcolor{red}{emulates} to extract all the \texttt{(Aspect, Opinion, Sentiment)} triplets from an unstructured text. %Despite performance progress, 
% contemporary ASTE approaches face challenges. 
% prior methods often rely on intricate frameworks, external information or heuristic enhancements, raising effectiveness and robustness concerns. Moreover, r

% 现状简介
% 当前的方法有两类，把ASTE看成理解问题或生成问题。其中，理解式多数基于PLM和分类头。

% 当前方法的诟病
% 但是，这些方法往往引入了过多不必要的复杂结构（分类头）或外部信息来达到更好的表现。

% 问题根源
% 本文认为问题的根本在于PLM的圆锥形上下文表征和tagging scheme不够精简导致的分类头难学。
%%这是由于大多数基于PLM的方法忽视了PLM圆锥形上下文表征的问题，且采取了不够精简的tagging scheme，从而增加了分类头学习的难度。

% Recent methods commonly utilize pretrained language models (PLMs) to encode input text. However, most PLM-based methods have long neglected the conical embedding distribution issue. 

% 本文的贡献
% 基于理论分析，我们重新设计了tagging scheme，其不仅采取了目前为止可比方法中最少的标签分类，从而易于分类头分类，而且在此基础上进一步设计了一种对比学习，从而改进了PLM输出词向量的分布。

% of disregard the cone-shaped embedding distribution issue, constraining PLMs' potential in downstream tasks and hence relying on intricate techniques to leverage the performance, including but not limited to complex architecture design and external information enhancements.

% 结果
% 经过这样的改进，我们方法在更小的分类头设计、更低开销的基础上取得了可比甚至高于sota的表现，为解决ASTE问题提供了本质的思考。

% GPT 时代的问题
% 值得注意的是，即使在大语言模型时代，我们的方法仍被证明在精确度和效率上超过GPT3.5和4的表现。

% 本文贡献
% 在本文中，我们采取了

% To address these issues, we propose a framework that combines two designs: 1) an innovative token-level contrastive learning strategy based on 2) an elegant novel tagging scheme. 
% The tagging scheme facilitates classification by employing a full matrix to locate, align and classify the pairs of \texttt{Aspect} and \texttt{Opinion} terms simultaneously while minimizing label classes. The contrastive learning mechanism leverages the \textit{uniformity} and \text{alignment} of representation distribution. 
% Experimental results shows that, though employing only a single classification layer, our method surpasses or compare favourably with the existing state-of-the-art methods, which means that our method effectively exploits the PLM's potential while eliminating the need for complicated design of classification head or external information enhancement. 
% Notably, our approach also shows state-of-the-art performance on other ABSA subtasks and exhibits seamless adaptability to various information extraction endeavors.
\end{comment}


% \todo{
% \noindent
% \textbf{1, mention the LLM advances in this research field and compare the perfromances; even more, try to combine these two\\
% 2, contrastive learning must be aligned with the tagging-scheme, stress out these from begin to the end \\
% 3, should revise the expression of terms and math notations carefully\\
% 4, the literature should be well organized\\
% 5, improve the layout and figure expression\\
% }
% % 缩减篇幅
% % gpt 内容&逻辑
% % 更新数据 & 相关叙述
% % 
% }


\begin{comment}
    Aspect Sentiment Triplet Extraction (ASTE) is a burgeoning subtask within the domain of fine-grained sentiment analysis, which aims to extract all the (Aspect, Opinion, Sentiment) triplets from unstructured textual data. Existing approaches to ASTE can be broadly categorized into two paradigms: those treating it as an understanding problem and those treating it as a generation problem. The former predominantly leverage pre-trained language models (PLMs) and classification heads.

However, these approaches often introduce superfluous and intricate structures, such as additional classification heads or external information, in order to achieve improved performance. This paper posits that the fundamental issue lies in the conical context representation of PLMs and the lack of conciseness in the employed tagging scheme, resulting in challenges associated with learning the classification heads.

To address this concern, the paper presents a reimagined tagging scheme that, based on theoretical analysis, minimizes the number of labels, thereby facilitating the classification of the heads. Furthermore, a contrastive learning method is devised to enhance the distribution of word vectors produced by PLMs.

Through these innovations, the proposed methodology achieves performance levels comparable to, or even surpassing, the state-of-the-art techniques, while featuring a more streamlined classification head design and reduced computational overhead. These findings offer valuable insights for resolving the ASTE problem.

It is noteworthy that, even in the era of large-scale language models, the proposed approach demonstrates superior efficacy and efficiency when compared to GPT3.5 and GPT4. This underscores the continued relevance of our method as one of the premier solutions for ASTE in the era of large language models.


\end{comment}
% Aspect Sentiment Triplet Extraction (ASTE), an emerging fine-grained\footnote{Generally, sentiment analysis can be based on three levels, namely, document-based, sentence-based, and aspect-based \citep{jing2021seeking}.} sentiment analysis task \cite{pontiki2014novel, pontiki2015semeval, pontiki2016semeval}, intends to identify and extract all structured sentiment information from unstructured raw text \cite{peng2020knowing}. %, specifically reviews and user feedback
% This structured sentiment information is defined in the form of triplets \texttt{\{Aspect, Opinion, Sentiment\}}. 
% Specifically, an \texttt{Aspect} term is the word or phrase states an object being talked about, an \texttt{Opinion} term is the word or phrase that gives a qualitative description of the \texttt{Aspect}, and \texttt{Sentiment} is the sentiment polarity classified based on the context, which usually takes from a tertiary scale \texttt{\{Positive, Neutral, Negative\}}.

% For example, consider the sentence: ``The battery life is good, but the camera is mediocre. ''
% The extracted triplets would be: \texttt{\{battery life, good, Positive\}} and \texttt{\{camera, mediocre, Neutral\}}. Figure \ref{fig.example} illustrates another example. 



% As a fine-grained task, ASTE can be helpful in many downstream applications, such as dialogue generation \cite{liu2022robustly,wei2019emotion,wang2021unire} and recommendation systems \cite{{wang2022multi,zou2022multi},zhao2022multi}.

% These years, ASTE has garnered considerable interest. 
% The early works adopt a two-stage pipeline \cite{peng2020knowing,zhang2020multi}. However, pipeline methods may suffer from intrinsic error propagation, leading to performance constraints inherent to first-stage bottlenecks. 
% Subsequent methodologies shifts to a joint extraction paradigm, which extract the triplets in one stage. 
% % beginning with 1D sequence-labeling-based methods and transitioning to 2D table-filling-based methods. 
% Early joint extraction methods treats ASTE as a sequence labelling problem, where a 1D ``\texttt{B-I-O}'' tagging scheme is used \cite{xu2020position}. 

% However, the 1D tagging scheme is demonstrated to be not competent 
% % to the ASTE task, for its weakness 
% in some cases, for example, a sentence contains multiple triplets (one-to-many) or one word is contained by multiple triplets \cite{liang2023stage}.
% Later works \cite{wu2020grid,chen2021semantic,chen2022enhanced,liang2023stage,fei2022inheriting,zhang2022boundary} develop several 2D tagging schemes and treat triplet extraction as a table-filling problem, achieving magical performance progress. 
% With the booming evolution in Large Language Model, some works explore novel generative-based methods \cite{mao2022seq2path,chia2023domain,yang2023pairing,wang2022contrastive} and machine-reading-comprehension-based methods \cite{mao2021joint, chen2021bidirectional,liu2022robustly,zhai2022mrc}.

% Despite the diversity, an elephant in the room seems to be long neglected: while most of these methods adopt Pretrained Language Models (PLMs) to encode representation of words, there is inherent fault to directly fine-tune on such representations. Recent works \cite{liang2021learning} report that the PLM-encoded are clustered in a narrow cone space. This can be seen as going against the merits of \textit{uniformity} and \textit{alignment} \cite{wang2020understanding}, so that may deteriorate the representation capacity of word embedding \cite{liang2021learning}. 
% This issue may limit the PLMs to exert their potential on specific downstream tasks. 

% Besides, though the current 2D-labelling methods has largely enhanced the capacity of joint extraction, they also suffer from the following aspects:

% \begin{itemize}
%     \item \textbf{Redundancy} Most of the tagging schemes are too complicated, introducing too many labels to help \textit{locating} and \textit{labelling}, which make the feature harder to learn.
%     \item \textbf{Conflict} Some of the methods may be not competent in the troublesome cases, such as overlapping, span conflict, and terms with multiple words.
%     \item \textbf{External Information Dependence} To enhance the performance, external semantic labels are usually introduced. The fusion of internal and external information is often tricky, however the rich information inside the PLMs are left not taken full advantage.
%     \item \textbf{classification head-design Dependence} Most existing 2D-tagging-based methods relies on a elaborately designed classification head to boost performance, however we argue that the PLMs itself is complicated enough, we need not just ``gild the lily''. 
% \end{itemize}


%%%%%%%%%%%%%%%%%%%%NEW

% In existing methods, there is a tendency to employ complex classification head designs and leverage information gain techniques in order to achieve marginal improvements in performance. However, it is important to note that these approaches may introduce unnecessary complexity and deviate from the original objective. Hence, in this work, we aim to address these concerns by proposing a more streamlined approach that focuses on the fundamental aspects of Aspect Sentiment Triplet Extraction (ASTE). Our method prioritizes the concise representation of the tagging scheme and employs a contrastive learning approach to enhance the distribution of word vectors output by pre-trained language models. By adopting this approach, we achieve comparable or superior performance to state-of-the-art techniques, while maintaining a more principled and efficient framework.

% 贡献
% 总而言之，本文的贡献主要包括以下三方面：
% 1）重新审视了ASTE任务中的2D tagging scheme即table filling方法，分析了全矩阵相对于半矩阵的优势，并全矩阵中标签的功能分解为location 和 classification。尽我们所知，这是首次正式地分析tagging scheme并为更合理地设计提供指导的尝试。
% 2）根据以上分析，设计了一个极简主义的tagging scheme，采取了目前为止最少的标签种类，从而便于学习。尤其是，我们重新设计的tagging scheme中可以很自然地引入token-level的对比学习机制以改进PLM编码得到的上下文词向量表示分布的uniformity和alignment，以利于分类。
% 3）我们首次正式地考虑了大模型时代的ASTE，为GPT3.5-Turbo和GPT4-Turbo定制了incontext-learning方法，测试了一组baseline，这揭示了chatGPT在该任务上的能力，同时也表明，即使在大语言模型时代，我们的方法在效率和表现上都仍然是领先的。

% In this work, we proposed ContrASTE, a simple framework to issue the problems we positioned and leverage the performance of ASTE. Mostly, our proposed framework contributes in two aspects:

% \begin{itemize}
%     \item It provides with a more simple and concise tagging scheme, which utilizes a efficient full matrix to handle confusion problem and adopts fewer classes of labels to simultaneously \textit{locate} and \textit{classify}. This can be demonstrated and illustrated to benefit by solving the trouble of \textit{redundancy} and \textit{conflict}. 
%     \item It is well-combined with a novel token-level contrastive learning strategy to better exploit the rich semantic information and potential of PLMs. 
% \end{itemize}

% Thanks to this essential design, our method catches up or outperforms state-of-the-art on all the recognized ASTE datasets \cite{wu2020grid, xu2020position}, with significantly lower overheads as well as simpler architecture design. 



% GPT baseline



% Moreover, by taking better advantage of the PLM itself, our proposed method is free from external information augmentation or complicated classification head design.
% It is note-worthy that the two points are coherent rather than mutually independent. The tagging scheme we tailored organize tensors in a squared matrix where the calculation of contrastive loss can be directly and seamlessly.
